Amalur: Data Integration Meets Machine Learning

The data needed for machine learning (ML) model training, can reside in different separate sites often termed data silos. For data-intensive ML applications, data silos pose a major challenge: the integration and transformation of data demand a lot of manual work and computational resources. With data privacy and security constraints, data often cannot leave the local sites, and a model has to be trained in a decentralized manner. In this work, we present a vision on how to bridge the traditional data integration (DI) techniques with the requirements of modern machine learning. We explore the possibilities of utilizing metadata obtained from data integration processes for improving the effectiveness and efficiency of ML models. We analyze two common use cases over data silos, feature augmentation and federated learning. Bringing data integration and machine learning together, we highlight the new research opportunities from the aspects of systems, representations, factorized learning and federated learning.

==> 6relatedWorks.tex <==
\section{Related Work}
\label{sec:rw}
\rihan{break this into each section}
%  We first review  the existing data representation supporting LA factorization (Sec.~\ref{ssec:fml}) 
Machine learning has been applied to improve key operations of data integration such as schema matching \cite{ DBLP:journals/tois/AlserafiARC20, 10.1145/3318464.3389742}, data matching \cite{kopcke2010evaluation, das2017falcon, 9338287, 10.1145/3318464.3389742}. However, except for data cleaning \cite{krishnan2016activeclean, krishnan2017boostclean, 9458702}, little has been discussed in terms of using the key DI operations to facilitate machine learning \cite{dong2018data}, which is the goal of this paper. 
The group of works most related to our work, is  \emph{in-DB machine learning}.
% integration of machine learning to databases. % \subsection{Factorized ML over relational data}
\todo[inline]{some discussion about DIML papers, e.g., 7359925}

\para{In-DB machine learning}
\label{ssec:fml}
Integration of machine learning in relational databases has become one of the most important database research topics \cite{Makrynioti2019survey}. 
% \cite{kumar2017data, Makrynioti2019survey, zhou2020database}. 
A common solution is to link ML algorithms with databases via 
carefully crafted 
user-defined functions (UDFs). 
%New types of databases such as Array-based databases start to emerge, e.g.,  SciDB \cite{brown2010overview}. 
Another way is to extend the data types for vector/matrix  and SQL queries for ML models \cite{10.1145/3277006.3277013, 10.14778/3317315.3317323}. 
Recent systems propose new intermediate data presentations \cite{10.14778/3342263.3342633, DBLP:conf/cidr/KaranasosIPSPPX20} or even novel tensor-based data models \cite{boehmsystemds}.
A more fundamental line of research is to support the formal languages of both worlds, i.e., relational algebra and linear algebra \cite{kumar2015learning, chen2017towards, Khamis2020, wang2020spores, alotaibi2021hadad}.
% decompose ML algorithms \cite{9101671}
Notably, the above approaches mostly propose a representation as the data abstraction. In contrast, in data integration it is important to understand data sources and their relationships. Thus, although we have also applied matrix-based data abstraction ($D_1$, $D_2$ in Fig.~\ref{fig:allMs}b), our main contribution, i.e.,  three proposed matrices, are representations of \emph{dataset relationships}. Those capture the matching and 
redundancy for columns and rows from different data sources.

% \para{LA factorization over normalized data}
% \para{Representations of dataset relationship}  The term \emph{indicator matrix} has been proposed in \cite{kumar2015learning, chen2017towards} for primary   PK-FK-joinable or equi-joinable tables. They share similar ideas to ours in terms of using binary matrices to indicate the matches between rows from different tables. In our vision, the semantics of  indicator matrices are richer. Besides row-level matching of inner joins as discussed in \cite{kumar2015learning, chen2017towards}, we have also covered how users choose to combine the datasets, i.e., the table-level relationships such as outer join, left join, and union as shown in Table~\ref{tbl:4cases}.  Moreover, the declarative representations in our vision include  also mapping matrix and redundancy matrix. They preserve another two fundamental aspects of relationships among sources, i.e., source-to-target schema-level mapping and data redundancy.  It then leads to new  research challenges of LA rewriting, as discussed in Sec.~\ref{ssec:LAR}, and also broadens  future research directions, e.g., federated learning as discussed in Sec.~\ref{ssec:FL}\wenbo{dead ref}.



 
% Notably, 
% Yet, their matrix generation procedure is different from Alg.~\ref{alg:IMGen}. 
% In \cite{chen2017towards} it first joins the joinable attributes (not entire tables), removes duplicated rows, and gets the row numbers of $T$. In Alg.~\ref{alg:IMGen}, the key input is the data matching between source tables. Together with the source table relationship indicated by the schema mapping (e.g., outer join, inner join), we construct the indicator matrix \emph{on-the-fly} without fixing the dimension of $T$ from the beginning.
 

% Among the above various choices,  we are particularly interested in LA factorization , due to its similarity with our problem setting. 
% To avoid the data redundancy of large joins and compute the target table,
% % \emph{Morpheus} \cite{chen2017towards}  
% LA operators are factorized and pushed down to source tables. It often leads to a significant runtime efficiency boost.  
% Similarly,   to avoid materializing the instances of  mediated schema,  in  virtual data integration the
%  queries against mediated/target schema  are rewritten into the  queries over source schemata \cite{doan2012principles}. 

==> CostEstimation.tex <==
\subsection{Cost Estimation with Silos Characteristics}
% \setlength{\textfloatsep}{\textfloatsepsave}
\setlength{\textfloatsep}{0pt} 
\begin{algorithm}[tb]
	\caption{Amalur}
	\label{alg:all}	
	%	\setstretch{0.85}
	\DontPrintSemicolon
	\KwIn{ML model $\mathcal{L}$,  source tables $\mathbf{D}$, Mapping matrices $\mathbf{M}$, Indicator matrices $\mathbf{I}$
		\\{\bf Output}: ML result $R$}
	\SetKwBlock{Begin}{function}{end function}
	\tcp{non-factorizable}
	\If{$costEstimate(\mathbf{D}, \mathcal{L}, \mathbf{M}, \mathbf{I}) = false$}{
	     $D_T \gets materializeT(\mathbf{D}, \mathcal{M})$\label{alg:all:genT}\tcp{generate target table} 
				 
		$R \gets modelExe(\mathcal{L}, D_T)$
				 
		\Return $R$ 
    }
    \tcp{factorizable}
	$R \gets factorizedModelExe(\mathcal{L}, \mathbf{D},\mathbf{M}, \mathbf{I})$ 
	
	
	\Return $R$
\end{algorithm}
 
 
\begin{figure}[t]
% \begin{subfigure}{.3\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=.8\linewidth]{figures/Eva/col_overlap.png}  
%   \caption{Increase column overlap}
%   \label{fig:col}
% \end{subfigure}
\begin{subfigure}{.49\linewidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/Eva/row_overlap.png}  
  \caption{Increase row overlap}
  \label{fig:row}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{figures/Eva/mixed.png}  
  \caption{Increase column/row overlap}
  \label{fig:mixed}
\end{subfigure}
\vspace{-0.2cm}
\caption{Initial experiment results (parameter values: $r_{S_1}=r_{S_2}=30000, c_{S_1} = c_{S_1}= 100, c_X = 5000$)}
\label{fig:eva}
% \vspace{-0.5cm}
\end{figure}

In the case where target table materialization is allowed, a subprolem of in-database model factorization is cost estimation. 
That is, as shown in Alg.~\ref{alg:all}, we need to perform cost estimation, in order to choose between  ML factorization or target table materialization. 
The known factors are the row/column overlap ratio between joinable tables \cite{chen2017linear}. 
Below we show the preliminary experiments of using our LMM operator rewriting rule and the proposed two types of matrices in Sec.~\ref{sec:rewrite}. 


 

\para{Preliminary experiment results} In the first experiment of Fig.~\ref{fig:eva}a, we fix the column overlap (ratio of matched columns among all columns) between $S_1$ and $S_2$ as 0.2, and increase the row overlap. 
On top of  blue bars are the times of Amalur's performance boost compared to the baseline. 
Since materializing the target table costs more time, we observe the significant runtime improvements (max. 39 times) by applying our rewrite rule of LMM from Sec.~\ref{ssec:LAR}. In the second experiment shown in Fig.~\ref{fig:eva}b, we increase both row and column overlaps between $S_1$ and $S_2$, which causes the size of $T$ to decrease.
We discover that the boost of factorization becomes trivial when the source tables have high row and column overlap (and consequently $T$ is smaller).
% From the two experiments we can see that 

\para{Research question}
Factors such as source/target table sizes, row/column overlaps, and matrix density will affect whether the factorization of a given LA operator is necessary.
Therefore, designing a \emph{cost estimation} component that decides \emph{when} the factorization should be performed, is essential. 

\textit{$\mathcal{Q}_1$: Given the ML model $\mathcal{L}$,  source tables $\mathbf{D}$, Mapping matrices $\mathbf{M}$, Indicator matrices,  how to estimate the cost and choose between factorization and materialization?}

$\mathcal{Q}_1$ can be extended with other possible factors, e.g., constraints of memory limit, data privacy rules. 


==> dataDiscovery.tex <==
%----------------------------Refs-----------------------------------%
% Seeping Semantics: Linking Datasets Using Word Embeddings for Data Discovery" in ICDE 2018. 
% Creating Embeddings of Heterogeneous Relational Datasets for Data Integration Tasks" in SIGMOD 2020.

\label{sec:discovery}

\para{Capturing relatedness among datasets} For Amalur to leverage from its LA rewriting, it needs to maintain information about potential  correspondences among columns of the heterogeneous tabular data residing in the data lake; this is made possible through the \textit{data discovery} component. With Amalur, we want to advocate novel approaches to the data discovery problem in data lakes, which could ameliorate the shortcomings of existing solutions (e.g. approximation through, possibly storage heavy, LSH indexes \cite{DBLP:conf/icde/FernandezAKYMS18}, non-scalable and possibly ineffective dataset discovery solutions \cite{Nargesian2018, zhang2020finding}). One such possible approach can be found in the recent attempts to revive and facilitate the use of state-of-the-art schema matching methods for capturing relevance among columns of tabular data, like in Valentine \cite{DBLP:conf/icde/KoutrasSIPBFLBK21:short, Koutras2021demo}. In short, Valentine consolidates some of the best efforts in schema matching, offering a scalable and easy-to-employ system for performing data discovery. Consequently, it seems to be a perfect fit for the needs of Amalur, since it offers a variety of methods that can help cover a wide spectrum of possible relevance types that we want to capture in a data lake. Another opportunity for Amalur's data discovery component, would be to incorporate modern embedding techniques in order to discover similar data elements. As we discussed in Sec. \ref{ssec:prof}, there are multiple embedding methods that our data discovery module can utilize, together with specific benefits and disadvantages. However, while using embeddings for capturing semantically-deeper relationships among data seems to be a very promising direction, we believe that, for the moment,  embedding-based data discovery should only be used in conjunction with other existing solutions; further improvements are needed in order to solely trust such methods for finding related datasets in a data lake system \cite{DBLP:conf/icde/KoutrasSIPBFLBK21:short}.


==> embOpps.tex <==
\subsection{Embeddings}
\label{sec:emboppo}
 
With Amalur, we opt for embedding cell values and columns of ingested tables into a high-dimensional space, which paves the way for capturing relevance among various datasets. However, there exist multiple embedding methods in the literature from which Amalur could benefit; hence, here we briefly discuss about the benefits/shortcomings of certain, widely-used embedding techniques and comment on their suitability for deployment in our data lake system.

\para{Pre-trained models} The simplest way to relate data elements, such as table columns, to vectors of a given dimensionality is to apply methods widely used for producing \textit{word embeddings} in  Natural Language Processing (NLP). Such methods, like Word2Vec\cite{mikolov2013distributed} and fastText \cite{bojanowski2017enriching}, offer pre-trained models on large amounts of natural language text, which can be applied to embed string values. Despite their seamless employment for embedding cell-values, and consequently table columns \cite{fernandez2018seeping, Nargesian2018}, pre-trained models have been shown to not generalize well on domain-specific datasets \cite{DBLP:conf/icde/KoutrasSIPBFLBK21:short}. Therefore, we believe that a data lake system that vastly depends on the effectiveness of its data discovery module, such as Amalur, should make use of more advanced embedding methods.

\para{Locally-trained skip-gram models} In order to deal with the limited generalization capability of pre-trained models, locally-trained embedding methods have emerged \cite{fernandez2019termite, cappuzzo2020creating}. In short, these methods leverage the architecture of \textit{skip-gram models} \cite{mikolov2013distributed, bojanowski2017enriching} used in NLP for training on large natural language corpora, in order to apply them on tabular data by making the necessary assumptions and adding data pre-processing steps. Whereas training on the tables residing in a data lake can be an improvement with respect to simply using pre-trained models, locally-trained models still seem to be insufficiently effective when used for matching related columns \cite{DBLP:conf/icde/KoutrasSIPBFLBK21:short}, due to the shortcomings of the training data construction process (lack of syntax as in the case textual data, non-holding assumptions on the format of real-world tabular data). In addition, such models require a lot of time and resources for constructing the training data, while they need retraining when there are changes on the datasets (additions/updates/deletions). Thus, employing them in a data lake system where we have continuous data updates, could considerably harm efficiency. Finally, mapping every data element (cell values, columns) to a vector representation could lead to an undesired storage overhead \cite{fernandez2019termite}.

\para{Locally-trained transformers} Recently a new line of work proposed the use of \textit{transformer} architectures, such as BERT \cite{devlin2018bert}, for embedding tabular data \cite{tang2020rpt, deng2020turl, yin2020tabert}. Transformer architectures tackle the shortcomings of the previous skip-gram based models, by introducing methods to embed similarly formatted data elements into different vectors with respect to the context they are found in the training data. This makes them more suitable in the case of data lakes, since same values in different tables might have different meanings with respect to the entities they refer to (e.g. the value 2021 can either refer to a year or an amount of money). Nonetheless, these methods still suffer from the training data construction problems that we mentioned in the previous paragraph, hence a data discovery system that encompasses them for generating embeddings could still be insufficiently effective and highly inefficient.

\para{Graph neural networks} All previous embedding methods have something in common: they need no supervision in order to be trained, since training samples are automatically constructed from the input. While this saves on costly human interference, it essentially limits effectiveness of the data discovery systems that utilize these embedding techniques in order to find relevant data. Recently, \textit{Graph Neural Networks} (GNNs) \cite{wu2020comprehensive} have gained a lot of popularity due to their straightforward applicability and surprising results in traditional problems such as \textit{classification} and \textit{link prediction}. GNNs benefit from the features of the nodes and the relationship information among them in the graph in order to build generalizable models that can be applied to unseen data during the training process. In essence, with GNNs we learn a ``recipe" to incorporate the neighborhood information and the features of each node in order to embed it into a vector. Therefore, by using a GNN-based embedding model (e.g. GraphSAGE \cite{hamilton2017inductive}) in a data lake system such as Amalur, we no longer need to pay the costs of retraining due to constant changes in the residing datasets. Yet, for generating high quality embeddings that lead to effective data discovery, we need to have in our possession a small portion of representative connections that hold among corresponding elements of disparate datasets. Nevertheless, the cost of incorporating humans in order to get training data to feed GNNs can be significantly less than the cost of constructing and maintaining the training data of the models we discussed above. Consequently, we aspire Amalur to engage a GNN-based embedding generation process, which will substantially boost the efficiency and effectiveness of data discovery. 
%To use standard machine learning algorithms on vector representations of data for computing distance, we need embeddings. For a particular task (e.g., data discovery) or a pipeline of data processing tasks, 
%can we find a universal method for embedding generation? 
%How shall we choose between pre-trained embeddings and local embeddings?
%To which extent the embedding should be stored? And which part better to be generated on-the-fly to avoid the storage cost and retraining cost?
% 0. check below survey
% J. Qin, W. Wang, C. Xiao, and Y. Zhang. Similarity query processing for
% high-dimensional data. PVLDB, 13(12):3437–3440, 2020.

% 1. pretrained embedding seems to be more approapite for NLP, thus record linkage.

% 2 do we want to claim about integration of images, videos through embeddings?

==> evaluation.tex <==
\section{Evaluation}
%PROTOTYPE SYSTEM EVALUATION
\label{sec:eva}


==> existing.tex <==
\section{Shortcomings of existing approaches}

\color{red}
From the notes yesterday:
\color{black}


Traditional data integration is made for answering queries via rewritings, or data exchange, and it has not been used for optimizing ML pipelines. This means that the existing cost models do not account for ML workloads. We need to revisit those.

(Want to manage data and train over silos under possible privacy constraints.)
Federated learning does not deal with data integration - they assume it. Moreover, FL works consider very primitive data matchings (key-key) - limits the usability / applicability. They consider only row matching (a limited version based on row IDs) while column mappings are not considered at all (Rihan to give input). 

Data integration is actually used as a pre-processing step and separates itself from ML. 

No unified data/processing architecture that combines data integration and ML, missing out on a lot of optimization opportunities.

==> opportunities.tex <==
\section{Opportunities}
\label{sec:oppo}
In this section we discuss the wide-open possibilities based on Amalur. 

\subsection{Native support of common ML tasks}
\label{ssec:LARopps}
% lead author: Rihan
% To what extent do we talk? a
% a. diverse relatedness   relationships between datasets in a lake
% b. nested tgds
% c. approximate FDs
% While automatically rewriting LA or even hybrid of LA and RA querying interface request, we need to consider the generality, equivalence, efficiency.
 {\color{green} Lead author: Asterios}
 
 
\textbf{Cost estimation.} Following the discussion in Sec.~\ref{ssec:LARopps} and \ref{ssec:LAR}, 
how the datasets are related (e.g., unionable, joinable), row/column overlap, size of source/target tables. 

\textbf{Relaxed relationships of datasets in data lakes.}
Datasets in a data lake are loosely integrated. 
That is, via data discovery we know the top-k datasets related to a given data set. 
And the relatedness often comes with a similarity score between each pair of attributes from different datasets. 
In our current approach we still assume the case that the data scientists will choose the additional datasets from the top-k candidate list, and verify which attributes are actually related (i.e., represent the same real world entity). However, it would be interesting to see whether for LA rewrite we can directly apply the data discovery results, i.e., matched attributes with scores, rather than human verified matching attribute pairs. 
Furthermore, we have the embeddings of the ingested data, which could be useful information to the cost model for improving the LA rewriting process. 

\textbf{Blank space of logic-based methods.} Another challenge is to explore whether it is possible to facilitate more `automated' and more `efficient' rewriting rules using logic-based methods. 
In this work we only consider normalized data. However, for many machine learning models data scientists handle array-based data. Meanwhile, in Sec.~\ref{ssec:dsndsm} we mainly explained full tgds. Nested  tuple generating dependencies (nested tgd) \cite{kolaitis2020language} are the mapping formalism describing nested data (e.g., XML, JSON). 
Of course, from such nested data representation to matrices we still need to enforce the sequences between data entries.
It is blank space in existing works to study whether existing logical formalism such as nested tgds could help automate or improve the efficiency of LA execution or  downstream ML models in general.  







%\input{embOpps}




==> profile.tex <==
% \subsection{Profiling}
% \textbf{Profiling.}
\label{ssec:prof}
% \textcolor{mypink1}{Lead author: Andra}
% Notes from Rihan: 
% 1. one or two sentence to mention that data is ingested and stored in the data lake, then start with profiling
% 2. Which profiling tools are used? What does the profile of a dataset include (for data discovery, for LA rewrite)?
% 3. where (e.g., metadata repository) and how (e.g., in what form) is the profiling results stored?
% 4. If possible, please use the running example to explain, for better understanding of your points
%-------------------------------------------------------%
%---------------------recover later---------------------%
% The profiling step starts automatically after data ingestion. Amalur captures not only single column profiles such as cardinalities, data types, semantic data types and value distribution, but also inclusion dependencies used to discover the primary-key foreign-key constraints. Amalur uses open-source profiling tools, such as Metanome \cite{10.14778/2824032.2824086} and Sherlock \cite{hulsebos2019sherlock}, and built-in Python profiling techniques provided by pandas. We store all the profiles as properties of the nodes in a graph database where each node represents the attributes of the datasets. Finally, Amalur uses the profiles in the data discovery step and later in the LA rewriting phase. Moreover, we provide the single column profiles in the UI to offer a better understanding of the datasets for the users and to help them during the data cleaning step.
%-------------------------------------------------------%



==> rw.tex <==
\section{Related Work}
\label{sec:rw}
% my survey on data lake
% also check Nantia's survey
Data lakes and in-database ML are both broad areas. 
Recent surveys on data lakes \cite{zagan2020data, sawadogo2020data, hai2021survey} and in-database ML \cite{Makrynioti2019survey, zhou2020database} give a comprehensive and fine-grained introduction on the diverse solutions. 
Recent systems  such as SystemDS \cite{boehmsystemds}, TensorFlow Extended \cite{katsiapis2019towards},
MLow \cite{zaharia2018accelerating} and middlewares such as  Magpie \cite{jindal2021magpie} assist the full life circle of scalable data science.
Although also aiming to serve data science, 
Amalur contributes to the extracting the data  and supporting LA operators on top of existing data lake functions. 
Moreover, although Amalur has a  web-based UI similar to data preparation and transformation tools such as Trifacta\footnote{\url{https://www.trifacta.com/}}, 
it targets at heterogeneous sources, and tries to avoid target table materialization or at least generate the target table automatically from schema mapping and entity linkage results. 

Thus, here we focus on the following two aspects most relevant to Amalur: existing data lake prototypes designed for data science, and combination of linear algebra and logical formalism. 
\subsection{Data lake systems for data science}
A straightforward solution to build a scientific data lake, is to 
apply the open-source tools that support data preparation pipeline and ML-related tasks (e.g., model debugging). 
For instance,  Spark is applied to build the logistic regression model for sentiment analysis 
and Python  libraries (e.g., Matplotlib) for visualization in \cite{DBLP:conf/icde/MehmoodGCKBVTR19}.
A more sophisticated manner is to integrate the specific data science tasks into the design of data lake functions. 
First,   when profiling the datasets, a scientific data lake might need to extract information relevant to the data science tasks \cite{zhang2020finding, DBLP:conf/sigmod/BrackenburyLMEU18}, e.g., manage notebook variables, scientific topics of the experimental data. 
\emph{KAYAK} \cite{maccioni2018kayak} divides the process of   data preparation into atomic operations, then allows data scientists to optimize the whole pipeline of data preparation.
% Juneau \cite{DBLP:journals/pvldb/ZhangI19, DBLP:conf/cidr/IvesZHZ19, zhang2020finding} 
\emph{Juneau} \cite{zhang2020finding} 
extends computational notebooks (e.g., Jupyter) 
%(Jupyter, JupyterLab, Apache Zeppelin, or RStudio)  notebooks
and provides searching over similar datasets to improve common data science tasks, such as finding additional data for training or validation, and feature engineering.
%training/validation data augmentation, linking data, features extraction, and data cleaning. 
When users specify a desired target table via the user interface, 
% tabular data or nested data that can be easily unnested into relations
the system can automatically return a ranked list of tables, 
which might  be relevant to the given table. 


% In DB support of machine learning}
% \label{ssec: inDBML}
% \textbf{Short comparison with other systems.} SystemDS, Maggie, how ours going to be different

% check Morpheus p1224

\subsection{Integrated handling of RA and LA}
Besides Morpheous that we already introduced in previous sections, here we discuss more works supporting LA in RDBMSs. 
% SystemDS: federated/local tensors
AIDA \cite{d2018aida} and Lara \cite{lara2019} develop intermediate representation that supports LA; while SPOOF \cite{elgamal2017spoof} and SPORES \cite{wang2020spores} explores expressing linear algebras with relational algebras.
To support optimizing mixed workload of relational algebra (RA) and LA, HADAD \cite{alotaibi2021hadad} provides an intermediate representation that combines relational models and integrity constraints. 
% It encodes LA operators in the relational model and use tgds and Equality Generating Dependencies (EGDs) \cite{} for LA pipeline optimization. 
Note that HADAD also uses tgds, which are used to encode the LA pipeline for optimization; whereas in Amalur we use the tgds for representing the relationship between related datasets in a data lake.



% \subsection{Data management systems for DS}
% Trifacta, Feature stores(?)

==> usecase.tex <==
% \section{Problem definition}
% \label{sec:pre}
% We first introduce the mapping formalism to describe  data integration scenarios in Sec.~\ref{ssec:mapping}. In this work, we focus on two ML use cases, feature augmentation and federated learning. In Sec.~\ref{ssec:4cases} we 
% explain how we capture the dataset relationships in these use cases  with the mapping formalism.
% % Finally, 
% We analyze our goals in Sec.~\ref{ssec:rq}. In this work, by ``dataset'' we restrict ourselves to relational tables.
 
 
% To prepare for this, in Sec.~\ref{ssec:dsndsm}  we first introduce two of the most crucial components for data integration in data lakes, i.e., data discovery and schema mapping, together with the well-studied formal foundation of schema mappings. 

% to fulfill DI requirements in data lakes 

 













 








% \para{Problem analysis}
% \label{ssec:rq}
% Now we revisit the  question $Q$ raised in Sec.~\ref{sec:intro}. 
% Given data sources, a traditional data integration system performs: (1) schema matching \cite{RahmBernsteinSurvey}  or data discovery given massive datasets \cite{DBLP:journals/pvldb/Miller18, DBLP:conf/icde/FernandezAKYMS18, DBLP:conf/sigmod/ZhuDNM19, bogatu2020dataset, zhang2020finding}, and then generate schema mappings  from schema matching \cite{hernandez2001clio} or from data examples \cite{alexe2008muse, DBLP:conf/sigmod/AlexeCKT11}; (2)  data matching between rows of source tables
% % , which can be obtained via entity resolution 
% \cite{fellegi1969theory, tejada2001learning, 10.1145/3132847.3132949}.
 

% Notably, Table~\ref{tbl:4cases} 
% the four DI scenarios in can apply to more ML tasks or other
% as we visioned in Sec.~\ref{sec:intro}, 


